Single-Step Arbitrary Lagrangian-Eulerian Discontinuous Galerkin Method for 1-D Euler Equations

We propose an explicit, single step discontinuous Galerkin (DG) method on moving grids using the arbitrary Lagrangian-Eulerian (ALE) approach for one dimensional Euler equations. The grid is moved with the local fluid velocity modified by some smoothing, which is found to considerably reduce the numerical dissipation introduced by Riemann solvers. The scheme preserves constant states for any mesh motion and we also study its positivity preservation property. Local grid refinement and coarsening are performed to maintain the mesh quality and avoid the appearance of very small or large cells. Second, higher order methods are developed and several test cases are provided to demonstrate the accuracy of the proposed scheme.

==> makefile <==
MAINFILE=springer-paper
BUILD_DIR=tmp/release
DEBUG_BUILD_DIR=tmp/debug
ifndef VERBOSE
.SILENT:
endif

all:	${MAINFILE}.tex
	echo "Rendering ${MAINFILE}"
	latexmk -pdf -interaction=nonstopmode \
		-logfilewarnings- -quiet -shell-escape \
		-outdir=${BUILD_DIR} \
		-auxdir=${BUILD_DIR} \
		${MAINFILE}.tex > /dev/null 2> /dev/null
	cp ${BUILD_DIR}/${MAINFILE}.pdf ${MAINFILE}.pdf
	echo "${MAINFILE} Rendered..."

debug:	${MAINFILE}.tex
	echo "Rendering ${MAINFILE}..."
	latexmk -pdf -interaction=nonstopmode \
		-logfilewarnings- -quiet -shell-escape \
		-outdir=${DEBUG_BUILD_DIR} -gg -cd \
		-auxdir=${DEBUG_BUILD_DIR} \
		${MAINFILE}.tex
	cp ${DEBUG_BUILD_DIR}/${MAINFILE}.pdf ${MAINFILE}.pdf
	echo "${MAINFILE} Rendered..."

